When Code Smells Meet ML: On the Lifecycle of ML-specific Code Smells in ML-enabled Systems

Context. The adoption of Machine Learning (ML)--enabled systems is steadily increasing. Nevertheless, there is a shortage of ML-specific quality assurance approaches, possibly because of the limited knowledge of how quality-related concerns emerge and evolve in ML-enabled systems. Objective. We aim to investigate the emergence and evolution of specific types of quality-related concerns known as ML-specific code smells, i.e., sub-optimal implementation solutions applied on ML pipelines that may significantly decrease both the quality and maintainability of ML-enabled systems. More specifically, we present a plan to study ML-specific code smells by empirically analyzing (i) their prevalence in real ML-enabled systems, (ii) how they are introduced and removed, and (iii) their survivability. Method. We will conduct an exploratory study, mining a large dataset of ML-enabled systems and analyzing over 400k commits about 337 projects. We will track and inspect the introduction and evolution of ML smells through CodeSmile, a novel ML smell detector that we will build to enable our investigation and to detect ML-specific code smells.

==> Sections/ResearchMethod.tex <==
The following section presents the details of the study, highlighting the main goal and the relative research questions. Subsequently the process designed to address the research questions proposed is illustrated in Figure \ref{fig:enter-label} and detailed in the next sections. 

\subsection{Goal and Research Questions}
The study aims to explore and discover how AI-Specific Code Smells (AI-CS) are prevalent in AI-enabled systems when AI-CS are introduced and how AI-CS are introduced.
We formulated the specific goal through the GQM approach~\cite{caldiera1994goal} to address our goal.

\goal{

\textbf{Purpose:} Observe

\textbf{Issue:} the prevalence, the introduction and the removal 

\textbf{Object:} of AI-specific Code Smells in AI-enabled systems

\textbf{Viewpoint:} from the points of view of AI developers.

}

We planned to accomplish the described research goal, specifically addressing three research questions.

\resquestion{0}{What is the prevalence of AI-Specific Code Smells in AI-enabled systems?}

The investigation into the prevalence, specified in \emph{\textbf{RQ}$_0$}, of AI-specific code smells in AI-enabled systems aims to identify and address the most common issues in these systems.
By addressing this research question, we can determine which AI-CS are prevalent and evaluate whether finding ways to alleviate them is worthwhile.


\resquestion{1}{When the AI-Specific Code Smells are introduced in AI-enabled systems?}

Investigating the moment of introduction of AI-CS highlights the conditions and contexts that lead developers to do it. Therefore, \emph{\textbf{RQ}$_1$} aims to understand firstly if AI-CS are introduced when the AI projects are created or are introduced during the system's evolution.
The results aimed to answer \emph{\textbf{RQ}$_1$} could be used to understand the moment developers should focus on mitigating AI-CS.

\resquestion{2}{Why are AI-specific code smells introduced in AI-enabled systems?}

While the specific temporal conditions during the evolution of AI-enabled systems help to understand the specific moment that an AI-CS is introduced, it is necessary to extract information about the reasons that led the developers to update the system by introducing an AI-CS. So, \emph{\textbf{RQ}$_2$} aims to extract the actions developers do during the evolution of AI-enabled systems that are likely to provoke the introduction of AI-CS.

\resquestion{3}{When and how AI-specific code smells are removed in AI-enabled systems?}

\emph{\textbf{RQ}$_3$} focuses on the timing and methods employed to remove AI-CS.
This research question is motivated by the need to understand the strategies and circumstances under which developers address and eliminate AI-CS. 
By identifying the set of strategies that developers used to remove AI-CS, we aim to extract insights useful to define automatic refactoring strategies for AI-CS. 

\resquestion{4}{How do AI-specific code smells survive over time in AI-enabled systems?}

Finally, \emph{\textbf{RQ}$_4$} aims to observe the survival time of each AI-CS to identify the ones that persist in the project over time. The outcome of the analysis can be utilized to focus on detecting the AI-CS that exhibits greater endurance during the software project's maintenance activities.   


We will design our work using the guidelines by Wohlin \etal \cite{wohlin2012experimentation} and the ACM/SIGSOFT Empirical Standards\footnote{Available at: \url{https://github.com/acmsigsoft/EmpiricalStandards}}; in particular, we will use the \quoted{General Standard}, \quoted{Data Science}, and \quoted{Repository Mining} guidelines. All the material (\eg datasets and scripts) will be publicly available on an online appendix.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Sections/Figure/research_method.pdf}
    \caption{Process Designed for the study}
    \label{fig:enter-label}
\end{figure}

\subsection{Dataset Description and Project selection}

To perform our investigations, we want to use the NICHE dataset \cite{10174042} \ie a dataset that contains  \numNicheProjects AI-enabled systems released at the MSR conference '23. The motivations that drove us to select this dataset are multiple: first of all, the dataset contains only popular, active, and large commit histories projects \ie projects with over 100 stars on GitHub, with commits more recent to the 1 May 2020 and with at least 100 commits. These characteristics permit us not to select personal or inactive projects.
In the second place, the authors manually labeled the projects in two categories: \quoted{well}- and \quoted{not-well} engineered, according to eight dimensions using the framework released by Munaiah \etal \cite{10.1007/s10664-017-9512-6}. We want to select attribute dimensions related to system quality \ie the continuous integration dimension, and we want to perform a cross-sectional analysis between all the RQs to verify if there are differences in terms of smells between projects that implement and do not implement continuous integration mechanisms.

Table \ref{table:dimensions} shows the eight dimension metrics provided by NICHE with a sort description.

\begin{table}[!h]
\centering
   \resizebox{0.8\columnwidth}{!}{
    \begin{tabular}{|l|p{5cm}|}
    \rowcolor{arsenic}
    \textcolor{white}{\textbf{Dimension}} &     \textcolor{white}{\textbf{Description}} \\
    \hline
    Unit testing &  The project provides unit tests.\\
    \hline
   \rowcolor{gray10}Architecture & The project has a clear and well-defined architecture.\\
    \hline
    Documentation & The project provide a clear description, useful during maintenance activities. \\
    \hline
   \rowcolor{gray10} Issues & The contributors use GitHub issues to manage activities or to schedule tasks.  \\
    \hline
    Continuous Integration &  The project uses CI practices to release new versions.\\
    \hline
   \rowcolor{gray10} History & The project has continuously and frequently changed. It suggests that the repo is already active. \\
    \hline
    Community & The project has a large number of contributors.\\
    \hline
   \rowcolor{gray10} License & The project provides a license set appropriately. \\
    \hline
    \end{tabular}
    }
     \caption{Description of the eight dimensions of the dataset NICHE.}
     \label{table:dimensions}
\end{table}

We preliminary mined the dataset using a Python script to understand how many projects are active and to have an overall total number of commits. This operation is necessary because it is reasonable to suppose that some projects could be no longer available for some reason (repositories should be archived, some communities should be migrated to other version control systems, or some repositories should be moved from public to private, and so on).
At the end of this step, we identified \numActiveProjects projects available out of the \numNicheProjects provided by NICHE, and \numTotalCommits commits. Furthermore, to better understand the project's characteristics, we also calculated descriptive statistics. 

Table \ref{table:DescriptiveStatistics} shows the descriptive statistics on the variables \quoted{Stars}, \quoted{Commits}, and \quoted{Lines of Code}. 
\begin{table}[!h]
\centering
   \resizebox{0.8\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|}
    \rowcolor{arsenic}
    \textcolor{white}{\textbf{}} & \textcolor{white}{\textbf{Stars}} &  \textcolor{white}{\textbf{Commits}} &  \textcolor{white}{\textbf{Lines of Code}}\\
    \hline
        Min & 100.0 & 100.0 & 10\\
        \hline
      \rowcolor{gray10}  1st Qu. & 211.0 & 219.0 & 3829 \\
        \hline
        Median & 529.5 & 420.5 & 9235 \\
        \hline
      \rowcolor{gray10}  Mean & 1977.6 & 1306.9 & 24414 \\
        \hline
        3rd Qu. & 1641.0 & 1069.8 & 21845 \\
        \hline
     \rowcolor{gray10}   Max & 76838.0 & 90927.0 & 699513\\
    \hline
    \end{tabular}
    }
     \caption{Descriptive Statistics of the NICHE Projects.}
     \label{table:DescriptiveStatistics}
\end{table}

\subsection{Data extraction}
Once projects are downloaded, we aim to gather structural metrics using PyDriller with fine-grained granularity. Specifically, we want to configure PyDriller to extract the commit history for a project \textsc{P} belonging to the set of Active Projects. For each commit, C$_i$ $\in$ P, we intend to collect information on the total number of files, the number of removed and added files, the commit date, and the commit message. Subsequently, we will combine this information with the data extracted from \CodeSmile to conduct our analyses.

\subsection{AI-Specific Code Smells Detection}
 To achieve the objectives of this study, we plan to develop an AI-CS-specific detection tool, \CodeSmile.
This tool will analyze the Abstract Syntax Tree (AST) of code to gather information about statements and methods.
Notably, despite the clarity and specificity of AI-CS definitions provided by Zhang \etal~\cite{10.1145/3522664.3528620}, there is currently a lack of automated solutions for detecting these code smells. \CodeSmile aims to fill this gap and provide an automatic solution to detect AI-CS.
The tool will use rule-based conditions from the definitions of Zhang~\etal~\cite{10.1145/3522664.3528620} to effectively identify the presence of AI-CS in code.
As a result of the detection, the tool will report all the AI-CS identified with the relative position (defined by the file name and the line).

\CodeSmile will successively analyze each commit of AI projects to report all the information useful for analyzing the introduction, the survival time, and the removal of AI-CS. 

\subsection{Data Analysis}
The following section explains how we want to analyze the collected data to respond to our research questions.

\paragraph{\emph{\textbf{RQ}$_0$}: AI-specific Code Smells Prevalence}

\CodeSmile will be used for all the AI projects selected in the study.
Therefore, we will observe the distribution of prevalence of each AI-CS. Statistical descriptive metrics and plots will be employed to understand the characteristics of each distribution. Then, insights on the most prevalent AI-CS across the several projects will be provided. 
Additionally, prevalence results will be further enriched by mapping each identified AI-CS to the specific stage of an AI pipeline, utilizing the mapping framework established by Zhang~\etal~\cite{10.1145/3522664.3528620}.
This additional mapping step will enhance our understanding of AI-CS, revealing the most prone areas within the AI development pipeline.

\paragraph{\emph{\textbf{RQ}$_1$}:When AI-Specific Code Smells are introduced}
The results of the detection of \CodeSmile to detect AI-CS across several commits in AI projects will be used to understand when an instance of AI-CS is introduced. 
Firstly, the list of commits that identify the specific smell $s_i$ will be identified.
Each instance of AI-CS will be identified through the location (\ie using the project name, the filename, and the line). Moreover, considering that the filename or the path could change due to rename operations, we will assign a unique ID for each file based on the historical information and use it instead of the original path.

Given $C$ as the list of commits containing $s_i$ located in file $f_h$, analyzing each $C_t \in C$, we will verify if the smell $s_i$ is also present in the file $f_h$ in the previous commit $C_{t-1}$.

Specifically, we first consider if the commit $C_{t-1}$ does a change or not in the smelly file $f_{h}$.
If not, $C_t$ is the first commit introducing the specific smell $s_i$.

Otherwise, there are two cases to consider:
\begin{itemize}
    \item The instance of the smell  present in the file $f_{h}$ in the commit $C_{t-1}$ is different from $s_i$, so, $C_t$ is the first commit that introduces the smell $s_i$.
    \item A modification has been applied to the file $f_{h}$ in the commit $C_{t}$, so the instance of the smell present in $C_{t}$ is the same of $C_{t-1}$.
\end{itemize}

Consequently, we address the identification of the two specific cases by analyzing the similarity of the two instances of smells respectively in $C_{t}$ and $C_{t-1}$.
In detail, given the code related to the two instances of AI-CS, we will use a code similarity analyzer.
From the several techniques for code similarity analysis, we planned to use the FuzzyWuzzy tool\footnote{https://github.com/seatgeek/thefuzz}, as suggested by  Ragkhitwetsagul~\etal~\cite{ragkhitwetsagul2018comparison}, that uses the fuzzy string match method to analyze the similarity between two snippets of code.




\paragraph{\emph{\textbf{RQ}$_2$}: Why are AI-specific code smells introduced in AI-enabled systems?} 
After collecting the list of commits for each instance of AI-CS, a deeper investigation of the factors that lead to the introduction will be performed.
In detail, the commit message of each AI-CS introduction commit will be analyzed.
Therefore, we extract useful information from the commit message that explains the change's rationale. Afterward, the list of rationales will be extracted using the pattern-matching approach, as used by Tufano \etal~\cite{7817894} for analyzing why traditional code smells are introduced.
In detail, we extract the commit message that represents the specific rationale, starting from the key label set indicating the change operations used on several repositories described in \Cref{table:change_operations}.
Finally, we will analyze the co-occurrence of the rationale commit and the introduction of the AI-CS.
We will also analyze if the introducing commit acknowledges the presence of the AI-CS, resulting in a self-admitted AI-CS.
\begin{table}[!h]
\centering
    \begin{tabular}{|l|p{0.7\columnwidth}|}
    \rowcolor{arsenic}
    \textcolor{white}{\textbf{Tag}} &     \textcolor{white}{\textbf{Description}}\\
    \hline
    Bug fixing &  The commit aimed at fixing a bug.\\
    \hline
   \rowcolor{gray10}Enhancement & The commit aimed at implementing an enhancement in the system.\\
    \hline
    New Feature & The commit aimed at implementing a new feature in the system. \\
    \hline
   \rowcolor{gray10} Refactoring & The commit aimed at performing refactoring operations.  \\
    \hline
    \end{tabular}
     \caption{Description of the change operation tags that we want use for the rationale analysis}
     \label{table:change_operations}
\end{table}
\paragraph{\emph{\textbf{RQ}$_3$:}How AI-specific code smells are removed in AI-enabled systems?}
Once the set of AI-CS is listed for each commit, the removal analysis will be performed. 
Given a specific commit \textit{$C_t$} and a modified file $F_h$ $\in$ $C_t$, for each instance of smells $s_i$ $\in$ $F_h$, we will verify if the smell $s_i$ it was removed in the file $F_h$ in the commit $C_{t+1}$.

 Specifically, we first consider if the commit $C_{t+1}$ does a change or not in the smelly file $f_{h}$. If not, we consider the $C_{t+1}$ containing still the smell.  Otherwise, if the commit  $C_{t+1}$ does a change in the smelly file, 
we need to verify if the smell identified $s_j$ in the commit \textbf{$C_{t+1}$} is the same as the previous commit ($s_i$). 
%more instances are present, we can consider the smell removed. Otherwise,
 Therefore, if the smell instance $s_j$ appears at the same location (ID file and line number) as $s_i$, we consider that the two smells are the same; 
Otherwise, if the AI-CS instance is still present in the file $f_{h}$, but in a different line, there are two cases to consider:
\begin{itemize}
    \item The instance of the smell $s_{j}$ present in the file $f_{h}$ in the commit $C_{t+1}$ is different from $s_i$, so the instance of AI-CS  $s_{i}$ that was present in the commit $C_{t}$ has been removed.
    \item A modification has been applied to the file $f_{h}$ in the commit $C_{t+1}$, so the instance of AI-CS $s_{i}$ is still present but in a different line number of the same file $f_{h}$, but $s_j$ is the same instance of $s_i$.
\end{itemize}


\todoi{explain the method and put an example}

\paragraph{\emph{\textbf{RQ}$_4$:}Survival Analysis of AI-Specific Code Smells}
To understand the lifetime of each instance of AI-CS, it is necessary to collect information on how many commits, starting from introducing and removing commits, present the specific instance of AI-CS.
Therefore, as a result of the analysis of the previous research questions, we build the lifespan of each instance of AI-CS represented as the number of commits in which the AI-CS is present from the smell-introducing commit to the smell-removing commit.
The extraction of the lifespans allows for collecting information about the mean lifespan of each type of AI-CS and understanding how the smells survive over time.




\subsection{Public Availability of Data}
To ensure the replicability of this work and enable researchers to build upon our study, we will release all materials, including scripts and datasets, in an online appendix.

==> Sections/Results.tex <==
\paragraph{\emph{\textbf{RQ}$_1$}:When AI-Specific Code Smells are introduced}
The results of the detection of \CodeSmile to detect AI-CS across several commits in AI projects will be used to understand the differences in presence committed by commit. 
Firstly, the list of commits that identify the specific instance of AI-CS for the first time will be identified.
Given $C$ as the list of commits containing the specific AI-CS instance $s_i$ located in file $f_h$. For each $C_t \in C$, we will verify if the smell $s_i$ is present also in the file $f_h$ in the commit $C_{t+1}$.
Each instance of AI-CS will be identified through the location (\ie using the project name, the filename, and the line).

==> Tables/Method/pysmell_table.tex <==
\begin{table*}[t]
    \centering
    \caption{List of code smell detectable by Pysmell \cite{Chen2016PySmell}}
    \begin{tabular}{l l l}
    \toprule
    \emph{Smell Name} & \emph{Granularity Level} & \emph{Detection Rule}  \\
    \midrule
    Large Class  (LC)  & Class  & $LOC >= 200 or NOA+NOM >40$  \\ 
    Long Method (LM) & Function & $LOC >=100$\\ 
    Long Parameter List (LPL)  & Function & $PAR >=5$ \\

    Large Message Chain  (LMC)  & Expression  & $LMC>=4$  \\ 
    Long Scope Chaining (LSC) & Function & $DOCC>=3$\\ 
    Long Base Class List (LBCL)  & Class & $NBC>=3$ \\
     Useless Exception Handling (UEH)  & Code Block & $(NEC=1 and NGEC=1) or NEC = NEEC$ \\
    Long Lambda Function (LLF) & Expression & $NOC>=80$ \\
    Complex List Comprehension (CLC) & Expression & $NOL+NOCC >=4$ \\
    Long Element Chain (LEC) & Expression & $LEC>=3$ \\
    Long Ternary Conditional Expression (LTCE) & Expression & $NOC>=40$ \\
    \bottomrule
    \hline
\end{tabular}
    
    \label{tab:pysmell_table}
\end{table*}
